A detailed spectroscopic analysis of the open cluster NGC 5460

Within the context of a large project aimed at studying early F-, A- and late B-type stars we present the abundance analysis of the photospheres of 21 members of the open cluster NGC 5460, an intermediate age cluster (logt ~ 8.2) previously unstudied with spectroscopy. Our study is based on medium and high resolution spectra obtained with the FLAMES instrument of the ESO/VLT. We show that cluster members have a nearly solar metallicity, and that there is evidence that the abundances of magnesium and iron are correlated with the effective temperature, exhibiting a maximum around Teff=10500 K. No correlations are found between abundances and projected equatorial velocity, except for marginal evidence of barium being more abundant in slower than in faster rotating stars. We discovered two He-weak stars, and a binary system where the hotter component is a HgMn star. We provide new estimates for the cluster distance (720 +/- 50 pc), age (logt = 8.2 +/- 0.1), and mean radial velocity (-17.9 +/- 5.2 km/s).

==> Table_Non_Members.tex <==
\begin{table*}
\caption[ ]{Element abundances, in $\log(N_{X}/N_{\rm tot})$, of the analysed cluster member
stars. The estimated internal errors in units of 0.01\,dex and the number of lines selected 
for each element are given in parenthesis. For comparison, the last row shows the solar 
abundances by \citet{met05}. Abundances obtained from just one line have no error (-;1).}
\label{ngc5460 abn memb}
%\rotatebox{90}{
\scriptsize{
\begin{tabular}{lcccccccc}
\hline
\hline
Star & He & C & O & Na & Mg & Al & Si & S \\
\hline
HD~122983     & -2.00(-;1)    & 	      & -3.41(-;1)    & 	      & -5.22(-;1)    & -6.19(-;1)    & -4.41(-;1)    & 	      \\
HD~123097     & -0.90(-;1)    & 	      & 	      & 	      & -4.55(36;3)   & -5.85(-;1)    & -4.54(01;2)   & 	      \\
HD~123182     & -1.48(-;1)    & 	      & -3.41(-;1)    & 	      & -4.56(01;2)   & -5.43(-;1)    & -4.58(09;2)   & 	      \\
HD~123183     & 	      &  	      & -3.40(11;4)   & 	      & -4.30(16;3)   & 	      & -4.37(19;2)   & 	      \\
HD~123184     & -0.90(05;3)   & -3.47(-;1)    & -3.28(01;3)   & 	      & -4.35(16;5)   & -5.56(-;1)    & -4.39(10;4)   & 	      \\
HD~123201B    & -1.00(03;6)   & -3.60(-;1)    & -3.28(-;1)    & 	      & -4.29(10;5)   & -5.70(-;1)    & -4.52(01;2)   & 	      \\
HD~123202     &	              & 	      & 	      & 	      & 	      & 	      & -4.62(-;1)    & 	      \\
HD~123226     & -1.02(05;2)   & 	      & -3.41(01;2)   & 	      & -4.64(08;3)   & -5.77(17;2)   & -4.63(-;1)    & -4.77(17;6)   \\
HD~123269     & -0.98(-;1)    & 	      & 	      & 	      & -4.58(16;3)   & -5.76(-;1)    & -4.42(-;1)    & -4.45(-;1)    \\
CD-47~8868    & 	      & 	      & 	      & 	      & -3.80(-;1)    & 	      & -4.52(-;1)    & 	      \\
CD-47~8869    & 	      & -3.50(-;1)    & 	      & 	      & -5.27(16;2)   & 	      & -4.34(-;1)    & 	      \\
CD-47~8889    & 	      & 	      & 	      & 	      & -4.20(06;3)   & -5.52(-;1)    & -4.52(17;2)   & 	      \\
CD-47~8905    & 	      & 	      & 	      & 	      & -4.03(11;3)   & 	      & -4.26(09;2)   & 	      \\
CPD-47~6379   & 	      & 	      & 	      & 	      & -4.10(28;3)   & 	      & -4.77(45;2)   & 	      \\
CPD-47~6385   & 	      & -3.27(13;5)   & 	      & 	      & -4.28(02;3)   & -5.35(-;1)    & -4.71(24;2)   & 	      \\
UCAC~11104969 & 	      & -3.47(-;1)    & 	      & 	      & -5.11(32;2)   & 	      & -3.58(-;1)    & 	      \\
UCAC~11105038 & 	      & -3.38(14;3)   & 	      & -5.78(03;2)   & -4.86(07;3)   & 	      & -4.37(15;3)   & 	      \\
UCAC~11105106 & 	      & 	      & 	      & -6.13(06;2)   & -4.62(21;4)   & 	      & -4.09(21;2)   & 	      \\
UCAC~11105176 & 	      & -3.24(04;2)   & 	      & 	      & -4.45(03;3)   & 	      & -4.21(-;1)    & 	      \\
UCAC~11105213 & 	      & -3.49(12;3)   & 	      & -5.69(04;2)   & -4.87(06;3)   & 	      & -4.27(13;3)   & -4.37(-;1)    \\
UCAC~11105379 & 	      & -3.42(05;3)   & 	      & -5.84(05;2)   & -4.69(03;3)   & 	      & -4.37(09;3)   & -4.58(-;1)    \\
sun           & -1.11         & -3.65         & -3.38         & -5.87         & -4.51         & -5.67         & -4.53         & -4.90         \\
\hline
Star & Ca & Sc & Ti & V & Cr & Mn & Fe & Ni \\
\hline
HD~122983     & 	      & -7.48(20;4)   & -7.37(13;3)   & 	      & -5.27(14;19)  & 	      & -3.81(12;100) & 	      \\
HD~123097     & 	      & 	      & -7.31(10;2)   & 	      & -6.78(12;2)   & 	      & -4.60(05;12)  & 	      \\
HD~123182     & -5.29(-;1)    & 	      & -6.87(08;5)   & 	      & -5.90(23;9)   & -5.19(23;9)   & -4.20(14;60)  & 	      \\
HD~123183     & 	      & 	      & -6.51(-;1)    & 	      & -5.81(01;2)   & 	      & -4.37(22;11)  & 	      \\
HD~123184     & -5.77(-;1)    & -9.21(-;1)    & -6.88(14;8)   & 	      & -6.15(13;10)  & -6.10(-;1)    & -4.29(14;57)  & 	      \\
HD~123201B    & 	      & 	      & -6.54(18;5)   & 	      & -5.99(14;4)   & 	      & -4.47(14;20)  & 	      \\
HD~123202     &		      & 	      & 	      & 	      & -5.94(10;2)   & 	      & -4.50(07;5)   & 	      \\
HD~123226     & 	      & 	      & -7.27(-;1)    & 	      & -6.63(12;6)   & 	      & -4.75(15;54)  & -5.86(-;1)    \\
HD~123269     & 	      & 	      & -7.26(25;2)   & 	      & -6.48(13;9)   & 	      & -4.57(16;60)  & -5.76(-;1)    \\
CD-47~8868    & 	      & 	      & -7.04(15;2)   & 	      & -6.40(25;4)   & 	      & -4.25(21;13)  & 	      \\
CD-47~8869    & -5.35(-;1)    & -9.68(-;1)    & -6.67(08;2)   & 	      & -6.58(11;4)   & -6.82(-;1)    & -4.50(10;15)  & 	      \\
CD-47~8889    & 	      & 	      & -7.07(13;3)   & 	      & -6.16(09;5)   & 	      & -4.27(17;22)  & 	      \\
CD-47~8905    & 	      & 	      & -7.07(13;3)   & 	      & -6.16(09;5)   & 	      & -4.27(17;22)  & 	      \\
CPD-47~6379   & 	      & 	      & -7.12(22;4)   & 	      & -5.15(15;4)   & 	      & -4.20(23;27)  & 	      \\
CPD-47~6385   & -5.30(09;4)   & -8.81(04;3)   & -6.85(13;12)  & 	      & -6.04(09;17)  & -5.99(03;2)   & -4.38(09;59)  & -5.55(30;2)   \\
UCAC~11104969 & -5.69(17;4)   & -9.43(-;1)    & -7.48(32;5)   & 	      & -6.76(15;6)   & -6.34(08;3)   & -4.62(05;12)  & -5.65(65;5)   \\
UCAC~11105038 & -6.23(09;8)   & -9.17(19;3)   & -7.64(17;19)  & 	      & -6.50(15;16)  & -6.83(14;3)   & -5.08(13;91)  & -6.09(18;9)   \\
UCAC~11105106 & -5.67(07;8)   & -8.56(22;2)   & -7.44(14;10)  & 	      & -6.81(09;10)  & -6.83(08;3)   & -5.03(15;54)  & -6.04(04;3)   \\
UCAC~11105176 & -5.86(06;4)   & -8.82(11;2)   & -6.97(19;7)   & 	      & -6.33(08;10)  & -6.35(17;3)   & -4.80(12;61)  & -5.74(16;5)   \\
UCAC~11105213 & -6.03(25;19)  & -9.23(09;4)   & -7.16(04;13)  & 	      & -6.27(15;24)  & -6.75(22;5)   & -4.61(16;133) & -5.67(16;15)  \\
UCAC~11105379 & -5.89(14;15)  & -9.11(11;4)   & -7.22(05;15)  & -7.76(-;1)    & -6.39(12;22)  & -6.78(12;4)   & -4.74(16;129) & -6.11(18;14)  \\
sun           & -5.73	      & -8.99	      & -7.14	      & -8.04	      & -6.40	      & -6.65	      & -4.59	      & -5.81	      \\
\hline
Star & Cu & Zn & Sr & Y & Ba & Pr & Nd &  \\
\hline
HD~122983     & 	      & 	      & 	      & 	      & -8.64(-;1)    & -7.57(20;3)   & -7.43(10;8)   & 	      \\
HD~123097     & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
HD~123182     & 	      & 	      & 	      & -9.81(-;1)    & -9.09(-;1)    & 	      & 	      & 	      \\
HD~123183     & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
HD~123184     & 	      & 	      & -9.34(-;1)    & 	      & 	      & 	      & 	      & 	      \\
HD~123201B    & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
HD~123202     &		      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
HD~123226     & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
HD~123269     & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
CD-47~8868    & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
CD-47~8869    & 	      & 	      & 	      & 	      & -9.70(-;1)    & 	      & 	      & 	      \\
CD-47~8889    & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
CD-47~8905    & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
CPD-47~6379   & 	      & 	      & 	      & 	      & 	      & 	      & 	      & 	      \\
CPD-47~6385   & 	      & 	      & 	      & 	      & -8.17(11;2)   & 	      & 	      & 	      \\
UCAC~11104969 & 	      & 	      & 	      & -8.64(03;2)   & -8.55(-;1)    & 	      & 	      & 	      \\
UCAC~11105038 & 	      & 	      & 	      & 	      & -9.18(16;2)   & 	      & 	      & 	      \\
UCAC~11105106 & 	      & -6.79(-;1)    & 	      & 	      & -9.63(-;1)    & 	      & 	      & 	      \\
UCAC~11105176 & 	      & 	      & 	      & 	      & -10.10(-;1)   & 	      & 	      & 	      \\
UCAC~11105213 & 	      & -7.15(-;1)    & 	      & -9.64(16;3)   & -8.51(16;2)   & 	      & 	      & 	      \\
UCAC~11105379 & 	      & -7.75(-;1)    & 	      & -9.87(13;2)   & -9.35(16;2)   & 	      & 	      & 	      \\
sun           & -7.83         & -7.44         & -9.12         & -9.83         & -9.87         & -11.33        & -10.59        &               \\ 
\hline
\end{tabular}
}
%}
\end{table*}

